Word-Level Alignment of Paper Documents with their Electronic Full-Text Counterparts

We describe a simple procedure for the automatic creation of word-level alignments between printed documents and their respective full-text versions. The procedure is unsupervised, uses standard, off-the-shelf components only, and reaches an F-score of 85.01 in the basic setup and up to 86.63 when using pre- and post-processing. Potential areas of application are manual database curation (incl. document triage) and biomedical expression OCR.

==> block.tex <==
\begin{table*}[htbp]
\centering
\begin{small}
\begin{tabular}{l|l|l|l|l|l}
\multicolumn{1}{c}{Settings} & \multicolumn{1}{c|}{Score} & \multicolumn{2}{c|}{nxml2conv} & \multicolumn{2}{c}{nxml2scan}\\ 
\hline
\multirow{2}{*}{\texttt{20}}                           & $R\_nxml$ & $80.91$ & $\pm12.59$ & $80.45$ & $\pm07.89$ \\
                                                       & $R\_ocr$  & $56.78$ & $\pm06.40$ & $53.61$ & $\pm10.96$\\
\hline
\multirow{2}{*}{\texttt{20\_dehyp}}                    & $R\_nxml$ & $83.10$ & $\pm12.62$ & $82.76$ & $\pm07.67$  \\
                                                       & $R\_ocr$  & $58.31$ & $\pm06.63$ & $55.15$ & $\pm11.22$ \\
\hline                                                       
\multirow{2}{*}{\texttt{20\_pre}}                      & $R\_nxml$ & $81.49$ & $\pm12.68$ & $81.09$ & $\pm07.80$ \\
                                                       & $R\_ocr$  & $57.19$ & $\pm06.46$ & $54.03.$ & $\pm11.02$\\


\hline
\multirow{2}{*}{\texttt{20\_dehyp\_pre}}               & $R\_nxml$ & $83.68$ & $\pm12.72$ & $83.41$ & $\pm07.75$ \\
                                                       & $R\_ocr$  & $58.72$ & $\pm06.70$ & $55.58$ & $\pm11.30$\\
\hline                                                       
\multirow{2}{*}{\texttt{20\_dehyp\_pre\_forcednonrec}} & $R\_nxml$ & $85.48$ & $\pm12.86$ & $85.29$ & $\pm07.64$ \\
                                                       & $R\_ocr$  & $59.98$ & $\pm06.83$ & $56.83$ & $\pm11.46$\\
\hline                                                       
\multirow{2}{*}{\texttt{20\_forcednonrec}}             & $R\_nxml$ & $82.68$ & $\pm12.75$ & $82.28$ & $\pm07.85$ \\
                                                       & $R\_ocr$  & $58.02$ & $\pm06.55$ & $54.83$ & $\pm11.14$\\
\hline                                                       

\multirow{2}{*}{\texttt{zzz}}             & $R\_nxml$ & $.$ & $\pm.$ & $.$ & $\pm.$ \\
                                                       & $R\_ocr$  & $.$ & $\pm.$ & $.$ & $\pm.$\\
\hline                                                       

\end{tabular}
\end{small}
\caption{Alignment Scores (micro-averaged). Stddev based on n=$68$ individual scores.}
\label{tab:alignment_recall_overview}
\end{table*}


\begin{table*}[htbp]
\centering
\begin{small}
\begin{tabular}{l|l|l|l|l|l|l|}
\multicolumn{1}{c|}{\multirow{2}{*}{Pre/Post-Processing}}  & \multicolumn{3}{c|}{nxml2conv} & \multicolumn{3}{c|}{nxml2scan} \\ 
    &                        \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F} \\ 
\hline
  
\texttt{-}                          & $94.44$ & $76.41$ & $84.47$ & $92.82$ & $74.68$ & $82.77$ \\
\texttt{dehyp}                      & $94.52$ & $78.54$ & $85.80$ & $92.96$ & $76.93.$ & $84.19$ \\
\texttt{pre}                        & $94.44$ & $76.97$ & $84.82$ & $92.82$ & $75.27$ & $83.13$ \\
\texttt{dehyp + pre}                & $\textbf{94.53}$ & $79.10$ & $86.13$ & $\textbf{92.96}$ & $77.54$ & $84.55$ \\
\texttt{forcednonrec}               & $94.43$ & $78.08$ & $85.48$ & $92.81$ & $76.37$ & $83.79$ \\
\texttt{dehyp + forcednonrec}       & $94.52$ & $80.23$ & $86.79$ & $92.94$ & $78.64$ & $85.20$ \\
\texttt{pre + forcednonrec}         & $94.44$ & $78.65$ & $85.83$ & $92.81$ & $76.98$ & $84.16$ \\
\texttt{dehyp + pre + forcednonrec global} & $94.52$ & $\textbf{80.80}$ & $\textbf{87.12}$ & $92.95$ & $\textbf{79.28}$ & $\textbf{85.57}$ \\
\texttt{dehyp + pre + forcednonrec local}  & $94.48$ & $\textbf{80.80}$ & $87.11$ & $92.89$ & $\textbf{79.28}$ & $85.55$ \\


\texttt{bla + blubb}                & $.$ & $.$ & $.$ & $.$ & $.$ & $.$ \\

\hline                                                        
\end{tabular}
\end{small}
\caption{Alignment Scores (micro-averaged, N=$68$). All results using \texttt{pre\_compress=$20$}.}
\label{tab:alignment_scores_overview}
\end{table*}


%\multirow{2}{*}{--}  & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} &  $ 81.16 $ \\
%                     &  & &  &  &   &  &  $\pm 8.09$ \\

\multirow{2}{*}{--}  & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} &  $ 81.06 $ \\
                     &  & &  &   &  &  &  $\pm 8.11 $ \\ % exp_18_full
\hline
\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} &  $ 81.77 $ \\
                     &  & &  &   &  &  &  $\pm 8.03 $ \\ % exp_19_
\hline
\multirow{2}{*}{--}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} &  $ 81.06 $ \\
                     &  & &  &   &  &  &  $\pm 8.11 $ \\ % exp_20
\hline

\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} &  $  $ \\
                     &  & &  &   &  &  &  $\pm  $ \\ % exp_21
\hline
\hline

\begin{figure*}[p]
\centering
\frame{\includegraphics[width=.3\textwidth]{images/PMC2169525-15.fromorgpdf.LOCAL.small.png}}\hfill 
\frame{\includegraphics[width=.3\textwidth]{images/PMC2169525-15.foreground.LOCAL.small.png}}\hfill
\frame{\includegraphics[width=.3\textwidth]{images/PMC2169525-15.background.LOCAL.small.png}}
\caption{Three image renderings of the same page: Original PDF (DOI$_{CONV}$) (left), scanned print-out w/ manual markup (DOI$_{SCAN}$) (center), and extracted markup only (right).}
\label{fig:three_images_per_page}
\end{figure*}

%For quantitative evaluation of the system, we simply compute the \textbf{recall} for aligning the tokens in the PMC version to those in the OCR version, as $R_{PMC} = \frac{aligned}{|PMC|}$, where $aligned$ is the absolute number of tokens in PMC that could be mapped unambiguously to tokens in the OCR version, and $|PMC|$ is the absolute number of tokens in the PMC version. 
%We do not evaluate precision, as that would require manual inspection of the mappings in order to identify incorrect alignments. 
%Instead, we just assume that \emph{if} an alignment could be established with all contextual conditions and plausibility checks (e.g.\ token adjacency) in place, \emph{then} this alignment is most likely correct. 
%While this assumption is clearly not always met, it is a workable solution for gauging the effect of changes in pre- and post-processing settings (cf.\ below).  
%\noindent
%Note that this form of evaluation also assumes that a perfect OCR version contains exactly the same tokens as the PMC version.
%In reality, this assumption almost never holds, because, as mentioned in Section \ref{sec:intro}, the textual content of the PDF document (which was printed) and the full-text document differ in terms of e.g.\ meta data and, even more importantly, in terms of the bibliography / references section, which is excluded from the PMC version, but always contained in the OCR version. 
%As a result, recall can suffer from a negative bias if e.g.\ sections of the original paper are not captured in the OCR, or from a positive bias if the OCR document contains more (meta) data than the full text variant. 
%The latter is frequently the case


\begin{comment}
\begin{table*}[htbp]
\centering
\begin{small}
\begin{tabular}{l|l|l|l|l|l|l|}
\multicolumn{1}{c|}{\multirow{2}{*}{Pre/Post-Processing}}  & \multicolumn{3}{c|}{nxml2conv} & \multicolumn{3}{c|}{nxml2scan} \\ 
    &                        \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F} \\ 
\hline
  
\texttt{-}                          & $94.44$ & $76.41$ & $84.47$ & $92.82$ & $74.68$ & $82.77$ \\
\texttt{dehyp}                      & $94.52$ & $78.54$ & $85.80$ & $92.96$ & $76.93.$ & $84.19$ \\
\texttt{pre}                        & $94.44$ & $76.97$ & $84.82$ & $92.82$ & $75.27$ & $83.13$ \\
\texttt{dehyp + pre}                & $\textbf{94.53}$ & $79.10$ & $86.13$ & $\textbf{92.96}$ & $77.54$ & $84.55$ \\
\texttt{forced}               & $94.43$ & $78.08$ & $85.48$ & $92.81$ & $76.37$ & $83.79$ \\
\texttt{dehyp + forced}       & $94.52$ & $80.23$ & $86.79$ & $92.94$ & $78.64$ & $85.20$ \\
\texttt{pre + forced}         & $94.44$ & $78.65$ & $85.83$ & $92.81$ & $76.98$ & $84.16$ \\
\texttt{dehyp + pre + forced} & $94.52$ & $\textbf{80.80}$ & $\textbf{87.12}$ & $92.95$ & $\textbf{79.28}$ & $\textbf{85.57}$ \\
\texttt{dehyp + pre + forced (local)}  & $94.48$ & $\textbf{80.80}$ & $87.11$ & $92.89$ & $\textbf{79.28}$ & $85.55$ \\
%\texttt{bla + blubb}                & $.$ & $.$ & $.$ & $.$ & $.$ & $.$ \\
\hline                                      \end{tabular}
\end{small}
\caption{Alignment Scores (micro-averaged, N=$68$). All results using \texttt{pre\_compress=$20$} and \texttt{Bio.pairwise2.align.globalxx()} for alignment, except for the last one, which uses \texttt{Bio.pairwise2.align.localxx()}. Max.\ values are given in bold.}
\label{tab:alignment_scores_overview}
\end{table*}
\end{comment}

\begin{comment}
\begin{table}[htbp]
\centering
\setlength\tabcolsep{5.0pt} % default value: 6pt
\begin{tabular}{|c|c|c||c|c|c|c|c|}
\multicolumn{3}{|c||}{\rotatebox{0}{\textbf{Pre}}}   & \multicolumn{4}{c|}{\rotatebox{0}{\textbf{Post}}}  &
\multicolumn{1}{c|}{\textbf{Result}}\\
\hline
\rotatebox{90}{De-hyphenate}	& \rotatebox{90}{Join incorrect OCR splits} & \rotatebox{90}{Split incorrect OCR joins} & \rotatebox{90}{Force-align single same length}	&\rotatebox{90}{Force-align multi same length}	&\rotatebox{90}{Force-align single diff. length}	&\rotatebox{90}{Force-align multi diff. length} & \multicolumn{1}{c|}{\textbf{$R_{PMC}$}}\\
\hline
\multirow{2}{*}{--}  & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--} &  $ 81.04 $ \\
                     &  & &  &   &  &  &  $\pm 8.16 $ \\ % 
\hline
\hline
\multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} &  $ 84.27 $ \\
                     &  & &  &   &  &  &  $\pm 8.13 $ \\ % exp_21
\hline
\hline
\multirow{2}{*}{--}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} &  $ 83.57 $ \\
                     &  & &  &   &  &  &  $\pm 8.24 $ \\
\hline

\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{--} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} &  $ 84.28 $ \\
                     &  & &  &   &  &  &  $\pm 8.14 $ \\
\hline
\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} &  $ 84.27 $ \\
                     &  & &  &   &  &  &  $\pm 8.14 $ \\
\hline
\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} &  $ 84.27 $ \\
                     &  & &  &   &  &  &  $\pm 8.13 $ \\
\hline
\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} &  $ 84.15 $ \\
                     &  & &  &   &  &  &  $\pm 8.10 $ \\
\hline
\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} & \multirow{2}{*}{\checkmark} &  $ 84.02 $ \\
                     &  & &  &   &  &  &  $\pm 8.14 $ \\
\hline
\multirow{2}{*}{\checkmark}  & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{--} &  $ 84.00 $ \\
                     &  & &  &   &  &  &  $\pm 8.11 $ \\
\hline


%\checkmark & \checkmark & \checkmark & G & \checkmark & \checkmark & \checkmark & \checkmark & 84.347 $\pm$ 8.114\\
%\checkmark & \checkmark & \checkmark & L & \checkmark & \checkmark & \checkmark & \checkmark & 84.400 $\pm$ 8.094\\

\end{tabular}
\caption{Results of non-exhaustive ablation on $80$ OCR-PMC document pairs.}\label{tab:results_1}
\end{table}
\end{comment}


%Apart from that, token-level evaluation like this is rather strict, because it penalizes the system for missing small \emph{local} alignments which, however, do not affect the correctness on the global (page or document) level.


% Interesting and useful results and practical applications.
%For full-text XML documents like those found on , the situation is quite different. 
%What can be gained?
%The present paper describes a procedure for 
%Born-digital documents are not often used as subject to OCR.
%However, 1) some scientific papers are only available as paper, 2) they might contain important 'annotations', and 3) a document image is the most versatile form of content representation, so it seems useful to start 'reading' at that level. 
%The work is part of a project for extracting biomedial entities from scanned and OCRed PDFs. Aligning uncorrected OCR output to the correct text from the original publication is a way to produce training data in which images of expressions (extracted from PDF images) are labelled with their correct expressions, including cases of super- and subscripts, greek letters etc. which are problematic to OCR. 
%(These are weak spots of OCR, while the majority of scientific papers can be processed well with off-the-shelf OCR like tesseract.)
%Information Extraction from Paper-Based Annotations
%Printed paper copies are still commonly used as the basis of close reading, e.g.\ during document triage and information extraction for database curation. 
%In the course of this, readers often create annotations in the form of color highlighting of words, lines, or entire sections. 
%Automatically extracting this type of information from the paper documents requires 1) identification of highlighted regions in the scanned document image, and 2) extraction of the text in these regions. 
%If full-text is available, it will greatly improve the extraction quality, because word-aligned full text can be returned instead of OCR results.
%Motivation: Paper documents are often / mostly used as the basis of literature-based curation.
%Mapping might be interesting in both directions: 
%Find sth. in electronic version, look at it in conventional / PDF paper. 
%Why use scanned paper?
%----------------------
%Initially, work on scanned paper documents was started out of *neccessity*:
%SRK Papers contain manually applied highlighting that we want to preserve (see example).
%Actually, many SRK papers are also available electronically, the majority in PDF, a smaller subset in XML full text (from PMC).
%Where available, we use the XML full texts to improve / correct scanning results. 


%DB-to-document backprojection
%map/project an entry from the database 'back' to the section in the original document that it was extracted / curated from.

%*Main objective*: 
%Creation of training data for developing ML methods for DeepCurate (e.g. for automatically highlighting parts in the document)
%*Side objective*: 
%Enrich SRK data entries with original context of extraction, for db users, but also as a means of quality assurance.

%Similar to EPMC 'SciLite' annotations, which, however, single out and link to entire verbatim passages.


%Bootstrapping!

%Make that a *virtue*:
%- paper is the preferred medium for manual curation

\noindent
%An inspection of a random sample of the OCR result returned by the service provider, however, showed that it was not satisfactory, mainly because it only provided word-level (as opposed to character-level) bounding boxes, and no recognition confidence scores.
%Therefore, it was decided to discard this data and to do the OCR processing from scratch.

%Instead, our algorithm combines the facts that 1) highlighting is always \emph{non-grey} and 2) shades of grey in the RGB color model are characterized by identical, or at least highly similar, values in the R, G, and B components.\footnote{https://en.wikipedia.org/wiki/Grey}

%\footnote{Version 1.7 or later is required for aligning \emph{lists of strings} (rather than \emph{strings of characters}.)} 
%, i.e.\ tuples with identical tokens will be aligned, while non-identical ones (no matter how \emph{similar} their tokens might be) will not be aligned. 


%a dictionary with OCR token ids as keys and (sequences of) PMC token ids as values.
%The choice of $n$ has to be small enough to allow for a considerable number of matches, otherwise the compression ratio will not be sufficient.
%On the other hand, $n$ needs to be large enough to avoid finding many repeated matches.


\begin{table*}[htbp]
\centering
\begin{small}
\begin{tabular}{l|l|l|l|l|l|l|}
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Pre/Post-Processing}}}  & \multicolumn{3}{c|}{\textbf{DOI$_{xml}$ -- DOI$_{conv}$}} & \multicolumn{3}{c|}{\textbf{DOI$_{xml}$ -- DOI$_{scan}$}} \\ 
    &                        \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c|}{F} \\ 
\hline
\texttt{-}                                  & $99.14$ & $80.21$ & $88.68$ & $98.86$ & $79.53$ & $88.15$ \\
\texttt{dehyp}                              & $99.15$ & $80.94$ & $89.12$ & $98.89$ & $80.37$ & $88.67$ \\
\texttt{pre}                                & $99.15$ & $80.75$ & $89.01$ & $98.86$ & $80.11$ & $88.51$ \\
\texttt{dehyp + pre}                        & $\textbf{99.17}$ & $81.48$ & $89.46$ & $98.90$ & $80.97$ & $89.04$ \\
\texttt{post\_force\_align}                 & $99.14$ & $81.96$ & $89.74$ & $98.87$ & $81.35$ & $89.26$ \\
\texttt{dehyp + post\_force\_align}         & $99.15$ & $82.71$ & $90.18$ & $98.90$ & $82.21$ & $89.79$ \\
\texttt{pre + post\_force\_align}           & $99.15$ & $82.52$ & $90.07$ & $98.87$ & $81.96$ & $89.62$ \\
\texttt{dehyp + pre + post\_force\_align}   & $99.16$ & $\textbf{83.26}$ & $\textbf{90.52}$ & $\textbf{98.91}$ & $\textbf{82.83}$ & $\textbf{90.16}$ \\
\texttt{dehyp + pre + post\_force\_align (local)}  & $99.12$ & $\textbf{83.26}$ & $90.50$ & $98.85$ & $\textbf{82.83}$ & $90.14$ \\
%\texttt{bla + blubb}                & $.$ & $.$ & $.$ & $.$ & $.$ & $.$ \\
\hline                                      \end{tabular}
\end{small}
\caption{Alignment Scores (micro-averaged, N=$68$). All results using \texttt{pre\_compress=$20$} and \texttt{Bio.pairwise2.align.globalxx()} for alignment, except for the last one, which uses \texttt{Bio.pairwise2.align.localxx()}. Max.\ values are given in bold.}
\label{tab:alignment_scores_overview}
\end{table*}

%The goal of these experiments is to provide an idea of the overall performance of the system and of the contributions of the individual pre- and post-processing steps.

%The expectation is that the results for the latter data are worse because 
%The first row shows the baseline result using only the alignment, which is $R_{PMC}=81.04$. 
%The second row shows the result with all pre- and post-processing heuristics active, which is $R_{PMC}=84.27$. This corresponds to a $4\%$ improvement. 
%The next rows show ablation results for the individual heuristics. The strongest effect can be seen in the third row, where removing the \textbf{De-hyphenate} heuristic causes the result to drop $0.7$ points. In all other cases, no single heuristic has a comparably strong effect. 


%briefly puts this application-oriented paper into the context of some 

%This is necessary because using a binary matching scheme does not guarantee that only tuples with actually matching tokens will be aligned.

%Likewise, the OCR version can contain tokens that were incorrectly joined.
%We identify these in a process that is the inverse of the one described above, i.e.\ we move a window of size $2$ over the list of PMC tuples and create merged words by concatenating the two tokens. 
%We then iterate over all tokens in OCR, looking for all that match the reconstructed word (which we assume to be the result of an incorrect merge).
%For post-processing, the token lists have the same length due to padding entries (\texttt{<<GAP>>}) that were inserted by the alignment algorithm in order to bridge sequences of non-alignable tokens. 

%Another, equally important function of post-processing is that it identifies \emph{non-trivial} mismatches between OCR and PMC, which are important for the OCR data generation task.

%, etc.\ to detect and correct character- and word-level OCR errors. 
%In the area of business documents, page-level OCR is also applied on e.g.\ invoices \cite{katti2018,sage2020}. Here, the extraction of text is not required, and optimization focuses on numerical values and their positions.

%\noindent
%Our approach exploits the fact that many research papers are available both in a standard printable form (mostly PDF) and increasingly also in full-text XML format. 
%We identified \emph{three} use cases which can be seen as contributing to \emph{two} different, but converging, strands of research: 
%The first two use cases (cf.\ Section \ref{sec:intro}) are 1. manual database curation and 2. document \emph{triage}. Provided that a given document of interest is available in both formats, these two tasks can directly benefit from the proposed alignment, as described in the paper.
%The third use case, ground-truth data creation for biomedical expression OCR, is different in that it contributes to the more general task of information extraction from scanned biomedical documents. 

